Uncertainty-sensitive Activity Recognition: a Reliability Benchmark and the CARING Models

Beyond assigning the correct class, an activity recognition model should also be able to determine, how certain it is in its predictions. We present the first study of how welthe confidence values of modern action recognition architectures indeed reflect the probability of the correct outcome and propose a learning-based approach for improving it. First, we extend two popular action recognition datasets with a reliability benchmark in form of the expected calibration error and reliability diagrams. Since our evaluation highlights that confidence values of standard action recognition architectures do not represent the uncertainty well, we introduce a new approach which learns to transform the model output into realistic confidence estimates through an additional calibration network. The main idea of our Calibrated Action Recognition with Input Guidance (CARING) model is to learn an optimal scaling parameter depending on the video representation. We compare our model with the native action recognition networks and the temperature scaling approach - a wide spread calibration method utilized in image classification. While temperature scaling alone drastically improves the reliability of the confidence values, our CARING method consistently leads to the best uncertainty estimates in all benchmark settings.

==> tables/tbl_results_class_wise_ece_old.tex <==
%!TEX root = ../root.tex



\begin{table*}[]
%\begin{table*}[!htbp]
	\centering
	\scalebox{1.1}{
\begin{tabular}{ll|lll|lll}
	\toprule
	Annotation                                   & Recall   & MeanScore & DeltaAcc & ECE     & MeanScore & DeltaAcc & ECE     \\
	\midrule
	closing bottle                              & 67.65  & 88.97   & 21.33  & 24.12 & 68.39   & .74    & 12.62 \\
	closing door inside                        & 92.31  & 98.51   & 6.21   & 8.22  & 86.00   & -6.31  & 8.30  \\
	closing door outside                       & 81.82  & 93.55   & 11.73  & 20.97 & 86.86   & 5.04   & 19.81 \\
	closing laptop                              & 53.85  & 87.52   & 33.67  & 35.96 & 65.41   & 11.57  & 21.71 \\
	drinking                                     & 81.69  & 96.62   & 14.93  & 16.41 & 90.32   & 8.63   & 11.63 \\
	eating                                       & 86.42  & 93.26   & 6.84   & 9.33  & 80.99   & -5.43  & 5.75  \\
	entering car                                & 100.00 & 99.25   & -.75   & .75   & 91.31   & -8.69  & 8.69  \\
	exiting car                                 & 100.00 & 95.17   & -4.83  & 4.83  & 91.19   & -8.81  & 8.81  \\
	fastening seat belt                        & 90.00  & 96.08   & 6.08   & 6.91  & 88.36   & -1.64  & 7.24  \\
	fetching an object                         & 76.03  & 93.77   & 17.74  & 18.28 & 79.42   & 3.40   & 5.32  \\
	interacting with phone                     & 85.49  & 96.04   & 10.55  & 10.55 & 84.67   & -.82   & 3.28  \\
	looking or moving around  & 16.13  & 88.29   & 72.16  & 72.16 & 66.47   & 50.34  & 50.34 \\
	opening backpack                            & .00    & 98.82   & 98.82  & 98.82 & 82.69   & 82.69  & 82.69 \\
	opening bottle                              & 58.54  & 89.74   & 31.21  & 34.87 & 73.73   & 15.20  & 23.12 \\
	opening door inside                        & 81.25  & 93.51   & 12.26  & 12.26 & 81.18   & -.07   & 10.20 \\
	opening door outside                       & 100.00 & 100.00  & .00    & .00   & 98.16   & -1.84  & 1.84  \\
	opening laptop                              & 57.89  & 83.18   & 25.28  & 30.23 & 59.23   & 1.33   & 25.52 \\
	placing an object                          & 66.77  & 93.03   & 26.25  & 26.25 & 75.90   & 9.13   & 9.25  \\
	preparing food                              & 5.00   & 90.01   & 85.01  & 85.01 & 61.51   & 56.51  & 56.51 \\
	pressing automation button                 & 88.17  & 98.68   & 10.51  & 11.06 & 91.80   & 3.63   & 5.20  \\
	putting laptop into backpack              & 16.67  & 92.67   & 76.00  & 76.00 & 76.46   & 59.80  & 59.80 \\
	putting on jacket                          & 54.44  & 87.38   & 32.93  & 32.93 & 66.25   & 11.81  & 15.92 \\
	putting on sunglasses                      & 75.00  & 95.29   & 20.29  & 20.29 & 85.89   & 10.89  & 13.48 \\
	reading magazine                            & 92.93  & 98.58   & 5.65   & 6.09  & 93.35   & .42    & 2.87  \\
	reading newspaper                           & 94.47  & 97.32   & 2.85   & 4.19  & 87.68   & -6.79  & 7.40  \\
	sitting still                               & 95.10  & 97.96   & 2.86   & 2.86  & 93.84   & -1.26  & 1.84  \\
	taking laptop from backpack               & .00    & 85.25   & 85.25  & 85.25 & 70.08   & 70.08  & 70.08 \\
	taking off jacket                          & 60.00  & 86.68   & 26.68  & 31.75 & 64.15   & 4.15   & 17.50 \\
	taking off sunglasses                      & 41.18  & 88.05   & 46.87  & 46.87 & 68.86   & 27.68  & 29.20 \\
	talking on phone                           & 71.60  & 92.55   & 20.95  & 22.96 & 78.26   & 6.65   & 13.36 \\
	unfastening seat belt                      & 80.56  & 91.89   & 11.34  & 12.77 & 77.44   & -3.11  & 13.82 \\
	using multimedia display                   & 92.39  & 97.38   & 4.99   & 4.99  & 91.25   & -1.14  & 2.28  \\
	working on laptop                          & 86.86  & 94.33   & 7.48   & 9.51  & 85.67   & -1.19  & 3.89  \\
	writing                                      & 86.07  & 95.03   & 8.97   & 11.51 & 85.19   & -.88   & 3.39  \\
	\midrule
	Mean                                         & 68.71  & 93.36   & 24.65  & 26.32 & 80.23   & 11.52  & 18.61\\
\bottomrule

\end{tabular}
	}
	\caption{
	Fine-grained activity level results for different views and modalities and their combination (I3D model). 	
		%Fine-grained Activities Recognition results for all views for I3D. Random Baseline accuracy is $2.94$.
	% We show that even though the driver is mostly visible in the frame for each of our selected views, the camera position still plays an important role in the performance of our models. 
	}
	\label{tbl:class-wise}
	\vspace{-0.3cm}
	
\end{table*}

==> tables/tbl_results_classification_multi_view.tex <==
%!TEX root = ../root.tex



\begin{table}[!b]
%\begin{table}[!htbp]
	\centering
	\scalebox{1.1}{
	\begin{tabular}{ @{}l  c c c@{}   }
		\toprule
		Camera & \makecell{View} &\makecell{Validation}  &  \makecell{Test}\\ 
		\midrule
		\multirow{5}{*}{\parbox{1.8cm}{NIR \\Cameras}}
		& front top & 69.57 &63.64\\ 
		& right top & 65.16 &60.80 \\ 
		& back 		& 54.70 	& 54.34 \\ 
		& face view & 49.73 & 42.98\\
		& left top 	& 68.72 & 62.83\\
		%& combined &\underline{72.70} & \underline{67.17}\\
		%\multicolumn{2}{c|}{Combined}  & 72.7 & 67.17\\
		\midrule
		\makecell[l]{Kinect Color}&\multirow{3}{*}{right top}   & 69.50 & 62.95\\
		\makecell[l]{Kinect Depth}& & 69.43 & 60.52\\
		\makecell[l]{Kinect IR}& &72.90 & 64.98\\
		%Combined & & \underline{73.80} & \underline{68.51}\\
		%\multicolumn{2}{c|}{Combined}  &73.8 & 68.51\\
		\midrule
		\multicolumn{2}{l}{\hspace{-0.2cm}Score Averaging Ensemble~\cite{martin2019drive}}  &74.85
		 &69.03\\
		 \multicolumn{2}{l}{\hspace{-0.2cm}CARING -- Ensemble (ours)}  & \textbf{76.18}
		 &\textbf{72.49}\\
		
		\bottomrule
	\end{tabular}
	}
	\caption{
	Fine-grained activity level results for different views and modalities and their combination (I3D model). 	
		%Fine-grained Activities Recognition results for all views for I3D. Random Baseline accuracy is $2.94$\%.
	% We show that even though the driver is mostly visible in the frame for each of our selected views, the camera position still plays an important role in the performance of our models. 
	}
	\label{table:multi_view}
	\vspace{-0.3cm}
	
\end{table}

==> tables/tbl_results_reliability.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table}[b]
	\scalebox{0.72}{
	\begin{tabular}{ @{}l|cc|cc|cc|cc@{}}
		\toprule
		\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \multicolumn{2}{c|}{\textbf{NLL}} & \multicolumn{2}{c}{\textbf{$\Delta_{Acc}$}} \\
		& val & test & val & test & val & test & val & test \\ 
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} \\
		I3D \cite{carreira2017quo} & 20.1 & X & X & X & X & X & X & X \\
		P3D & X & X & X & X & X & X & X & X \\
		C3D & X & X & X & X & X & X & X & X \\
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}\\
		I3D + Temperature Scaling \cite{Guo2017} &	4.00& 7.75 & 26.08 & 17.34 & 0.81 &1.57& X & X \\
		CARING - I3D w.o. shuffle loss & 2.89 & 6.11 &  18.75 & 14.80 & 0.81 & 1.54 & X & X \\
		CARING - I3D  & 2.72 & 6.02 &  14.23 & 13.12 & 0.82  & 1.54 & X & X \\

%		\bottomrule

	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	\vspace{-0.3cm}
	\label{table:action_reco_objectlevel}
	
	
	

\end{table}



==> tables/tbl_results_reliability_hmdb51.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table}[b]
	\scalebox{0.72}{
	\begin{tabular}{ @{}l|cc|cc|cc|cc@{}}
		\toprule
		\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \multicolumn{2}{c|}{\textbf{NLL}} & \multicolumn{2}{c}{\textbf{$\Delta_{Acc}$}} \\
		& val & test & val & test & val & test & val & test \\ 
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} \\
		I3D \cite{carreira2017quo} & 20.1 & X & X & X & X & X & X & X \\
		P3D & X & X & X & X & X & X & X & X \\
		C3D & X & X & X & X & X & X & X & X \\
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}\\
		I3D + Temperature Scaling \cite{Guo2017} &	4.00& 7.75 & 26.08 & 17.34 & 0.81 &1.57& X & X \\
		CARING - I3D w.o. shuffle loss & 2.89 & 6.11 &  18.75 & 14.80 & 0.81 & 1.54 & X & X \\
		CARING - I3D  & 2.72 & 6.02 &  14.23 & 13.12 & 0.82  & 1.54 & X & X \\

%		\bottomrule

	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	\vspace{-0.3cm}
	\label{table:action_reco_objectlevel}
	
	
	

\end{table}



==> tables/tbl_results_reliability_pakos_ids1_ids1.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table*}[b]
	\scalebox{0.78}{
	\begin{tabular}{ l|cccccc|cccccc|cccccc}
		%\specialrule{.8pt}{2pt}{0pt}
		\toprule
		\multirow{3}{*}{\cellcolor{tablegrey} \textbf{Model}}& \multicolumn{6}{c|}{\cellcolor{lightsteellila}\textbf{All activity classes}} & \multicolumn{6}{c|}{\cellcolor{lightsteelblue} \textbf{Rare activity classes}} & \multicolumn{6}{c}{\cellcolor{lightsteelgreen} \textbf{Common activity classes}}\\ 
		 \cellcolor{tablegrey} \textbf{Model}&\multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{ECE}} &
		 \multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteellila}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteelblue}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{MCE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{NLL}} \\
		\cellcolor{tablegrey}&\cellcolor{lightsteellila} val &\cellcolor{lightsteellila} test &\cellcolor{lightsteellila} val & \cellcolor{lightsteellila}test & \cellcolor{lightsteellila}val & \cellcolor{lightsteellila}test  &\cellcolor{lightsteelblue} val &\cellcolor{lightsteelblue} test & \cellcolor{lightsteelblue}val &\cellcolor{lightsteelblue}test &\cellcolor{lightsteelblue} val & \cellcolor{lightsteelblue}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test & \cellcolor{lightsteelgreen}val & \cellcolor{lightsteelgreen}test  \\ 
		\specialrule{.4pt}{0pt}{2pt}
		%\hline
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} & & & & & & & & & & & & \\
		I3D \cite{carreira2017quo} & 13.68 & 15.95 & 50.95 &  49.08 & 1.05 & 1.31 & & & & & & & & & & & & \\
		P3D & X & X & X & X & X & X  & & & & & & & & & & & & \\
		%C3D & X & X & X & X & X & X  \\
		\midrule
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}& & & & & & & & & & & & \\
		I3D + Temperature Scaling \cite{Guo2017} &	7.12& 7.57 & 32.50 & 21.73 & 0.75 &0.96 & & & & & & & & & & & & \\
		CARING - I3D  & 5.12 & 6.95 & 26.87  & 46.38 & 0.73 & 0.94  & & & & & & & & & & & & \\


& & & & & & & & & & & &  \\
		\bottomrule
	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	
	\label{table:action_reco_objectlevel}
	
	
	

\end{table*}



==> tables/tbl_results_reliability_pakos_ids1_ids1_wide.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table*}[b]
	\scalebox{0.78}{
	\begin{tabular}{ l|cccccc|cccccc|cccccc}
		%\specialrule{.8pt}{2pt}{0pt}
		\toprule
		\multirow{3}{*}{\cellcolor{tablegrey} \textbf{Model}}& \multicolumn{6}{c|}{\cellcolor{lightsteellila}\textbf{All activity classes}} & \multicolumn{6}{c|}{\cellcolor{lightsteelblue} \textbf{Rare activity classes}} & \multicolumn{6}{c}{\cellcolor{lightsteelgreen} \textbf{Common activity classes}}\\ 
		 \cellcolor{tablegrey} \textbf{Model}&\multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{ECE}} &
		 \multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteellila}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteelblue}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{MCE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{NLL}} \\
		\cellcolor{tablegrey}&\cellcolor{lightsteellila} val &\cellcolor{lightsteellila} test &\cellcolor{lightsteellila} val & \cellcolor{lightsteellila}test & \cellcolor{lightsteellila}val & \cellcolor{lightsteellila}test  &\cellcolor{lightsteelblue} val &\cellcolor{lightsteelblue} test & \cellcolor{lightsteelblue}val &\cellcolor{lightsteelblue}test &\cellcolor{lightsteelblue} val & \cellcolor{lightsteelblue}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test & \cellcolor{lightsteelgreen}val & \cellcolor{lightsteelgreen}test  \\ 
		\specialrule{.4pt}{0pt}{2pt}
		%\hline
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} & & & & & & & & & & & & \\
		I3D \cite{carreira2017quo} & 13.68 & 15.95 & 50.95 &  49.08 & 1.05 & 1.31 & & & & & & & & & & & & \\
		P3D & X & X & X & X & X & X  & & & & & & & & & & & & \\
		%C3D & X & X & X & X & X & X  \\
		\midrule
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}& & & & & & & & & & & & \\
		I3D + Temperature Scaling \cite{Guo2017} &	7.12& 7.57 & 32.50 & 21.73 & 0.75 &0.96 & & & & & & & & & & & & \\
		CARING - I3D  & 5.12 & 6.95 & 26.87  & 46.38 & 0.73 & 0.94  & & & & & & & & & & & & \\


& & & & & & & & & & & &  \\
		\bottomrule
	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	
	\label{table:action_reco_objectlevel}
	
	
	

\end{table*}


